Learning Visual Information Utility with PIXER

Accurate feature detection is fundamental for various computer vision tasks, including autonomous robotics, 3D reconstruction, medical imaging, and remote sensing. Despite advancements in enhancing the robustness of visual features, no existing method measures the utility of visual information before processing by specific feature-type algorithms. To address this gap, we introduce PIXER and the concept of "Featureness," which reflects the inherent interest and reliability of visual information for robust recognition, independent of any specific feature type. Leveraging a generalization on Bayesian learning, our approach quantifies both the probability and uncertainty of a pixel's contribution to robust visual utility in a single-shot process, avoiding costly operations such as Monte Carlo sampling and permitting customizable featureness definitions adaptable to a wide range of applications. We evaluate PIXER on visual odometry with featureness selectivity, achieving an average of 31% improvement in RMSE trajectory with 49% fewer features.

==> sections/tables/eval.tex <==
% \begin{table}[htbp]
% % \vspace{0.5cm}
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}l|llll|llll|llll@{}}
% \toprule
% \multicolumn{1}{c|}{\multirow{2}{*}{Feature}} & \multicolumn{4}{c|}{KITTI}                          & \multicolumn{4}{c|}{CODa}                    & \multicolumn{4}{c}{Davis}            \\ \cmidrule(l){2-13} 
% \multicolumn{1}{c|}{}                         & RMSE           & MAE  & Time  & \(|kp|\downarrow\) & RMSE  & MAE   & Time   & \(|kp|\downarrow\) & RMSE  & MAE   & Time   & \(|kp|\downarrow\) \\ \midrule
% BRISK                                         & 1.782          & 1.17 & 42.26 &\phantom{0}                   & 46.64 & 34.27 & 109.97 &\phantom{0}                   & 31.44 & 20.50 & 141.28 & \phantom{0}        \\
% BRISK + Ours                                  & \textbf{1.547} & \textbf{1.27} & \textbf{40.32} & 54.4                & \textbf{46.33} & \textbf{30.64} & \textbf{106.56} & 68.2                & \textbf{15.74} & \textbf{9.52}  & \textbf{139.27} & 52.52       \\ \midrule
% FAST                                          & 2.631          & 1.91 & 37.08 &\phantom{0}                   & 9.37  & 4.42  & 64.88  &\phantom{0}                   & 12.04 & 6.40  & 148.98 & \phantom{0}        \\
% FAST + Ours                                   & \textbf{1.731}          & \textbf{1.48} & \textbf{33.66} & 44.1                & \textbf{4.39}  & \textbf{3.37}  & \textbf{54.47}  & 49                  & \textbf{3.59}  & \textbf{2.65}  & \textbf{138.33} & 32.26       \\ \midrule
% LOFTR                                         &                &      &       &\phantom{0}                   &       &       &        &\phantom{0}                   & 28.15 & 18.02 & 477.84 & \phantom{0}        \\
% LOFT + Ours                                   &                &      &       &                     &       &       &        &                     & \textbf{27.48} & \textbf{17.87} & \textbf{453.89} & 24.79       \\ \midrule
% ORB                                           & 1.802          & 1.27 & 42.09 &\phantom{0}                   & 47.1  & 30.8  & 78.59  &\phantom{0}                   & 14.46 & 8.30  & 209.12 & \phantom{0}        \\
% ORB + Ours                                    & \textbf{1.469}          & \textbf{1.03} & \textbf{39.58} & 45                  & \textbf{35.58} & \textbf{22.9}  & \textbf{71.54}  & 68.7                & \textbf{10.21} & \textbf{4.97}  & \textbf{200.97 }& 32.49       \\ \midrule
% SIFT                                          & 3.996          & 2.92 & 43.42 &\phantom{0}                   & 6.57  & 3.37  & 176.06 &\phantom{0}                   & 29.61 & 18.79 & 80.19  & \phantom{0}        \\
% SIFT + Ours                                   & \textbf{1.817}          & \textbf{1.49} & \textbf{42.58} & 57                  & \textbf{2.69}  & \textbf{1.88}  & \textbf{168.18} & 65.9                & \textbf{26.49} & \textbf{17.04} & 80.73  & 65.37       \\ \midrule
% Superpoint                                    & 1.745          & 1.41 & 45.83 &\phantom{0}                   & 4.29  & 2.43  & 125.93 &\phantom{0}                   & 30.53 & 20.02 & 145.73 & \phantom{0}        \\
% Superpoint + Ours                             & \textbf{1.188}          & \textbf{0.89} & 46.75 & 40                  & \textbf{2.03}  & \textbf{1.6}   & \textbf{124.41} & 43.1                & \textbf{29.43} & 20.89 & \textbf{140.04} & 36.18       \\ \midrule
% SURF                                          & 2.816          & 2.22 & 52.97 &\phantom{0}                   & 56.13 & 44.96 & 225.37 &\phantom{0}                   & 30.96 & 19.55 & 116.41 & \phantom{0}        \\
% SURF + Ours                                   & \textbf{1.218 }         & \textbf{1.07} & \textbf{52.12} & 55.2                & \textbf{38.49} & \textbf{23.81} & \textbf{224.37} & 73.8                & \textbf{26.38} & \textbf{17.39} & 117.75 & 60.07       \\ \midrule
% LK\_SHI\_TOMASI                                 & 30.16          & 9.14 & 10.69 &\phantom{0}                   & 43.18 & 27.07 & 12.94  &\phantom{0}                   & 16.25 & 9.85  & 59.83  & \phantom{0}        \\
% LK\_SHI\_TOMASI + Ours                          & \textbf{3.66}           & \textbf{2.65} &\textbf{ 9.367} & 61.4                & \textbf{39.97} & \textbf{26.76} & \textbf{11.7}   & 68.7                & \textbf{10.23} & \textbf{7.40}  & 60.43  & 36.28       \\ \bottomrule
% \end{tabular}%
% }
% \caption{visual odometry performance results. Features when filtered using \qq{} contribute to a lower RMSE, MAE and execution time for visual odometry (VO) estimation. \(|kp|\downarrow\) is the avereage percentage reduction in the number of keypoints for each VO sequence.\task{add num keypoints columns, align decimals, same significant digits}\yash{time - vo time two columns} \task{recompute mean inference time if we have time}}
% \label{tab:vo-eval}
% \end{table}






% %% BACKUP

% \begin{table*}[]
% \resizebox{\textwidth}{!}{
% \begin{tabular}{@{}l|ccccc|ccccc|ccccc@{}}
% \toprule
% \multirow{2}{*}{Feature} & \multicolumn{5}{c|}{\textbf{KITTI} ($mean(F_\text{Area})$: 30.98\%)} & \multicolumn{5}{c|}{\textbf{CODa} ($mean(F_\text{Area})$: 33.65\%)} & \multicolumn{5}{c}{\textbf{Davis} ($mean(F_\text{Area})$: 66.21\%)}\\\cmidrule(l){2-16}
%  & \multicolumn{1}{l}{RMSE (m)} & \multicolumn{1}{l}{MAE (m)} & \multicolumn{1}{l}{Time (ms)} & \multicolumn{1}{l}{$mean (|KP|)$} & \multicolumn{1}{l|}{$mean (|KP|\downarrow)$} & \multicolumn{1}{l}{RMSE (m)} & \multicolumn{1}{l}{MAE (m)} & \multicolumn{1}{l}{Time (ms)} & \multicolumn{1}{l}{$mean (|KP|)$} & \multicolumn{1}{l|}{$mean (|KP|\downarrow)$} & \multicolumn{1}{l}{RMSE (m)} & \multicolumn{1}{l}{MAE (m)} & \multicolumn{1}{l}{Time (ms)} & \multicolumn{1}{l}{$mean (|KP|)$} & \multicolumn{1}{l}{$mean (|KP|\downarrow)$}\\\midrule
 
% BRISK & \phantom{0}1.78 & \textbf{\phantom{0}1.17} & \textbf{\phantom{0}60} & \phantom{0,}752.34 & \phantom{0} & 
%     46.64 & 34.27 & 116 & \phantom{00,}567.94 & \phantom{0} & 
%     32.63 & 23.92 & \textbf{\phantom{0}91} & 1,125.75 & \phantom{0} \\
% BRISK + Ours & \textbf{\phantom{0}1.55} & \phantom{0}1.27 & \textbf{\phantom{0}60} & \textbf{\phantom{0,}342.89} & 54.42 & 
%     \textbf{46.33} & \textbf{30.64} & \textbf{114} & \textbf{\phantom{00,}180.81} & 68.20 & 
%     \textbf{13.10} & \textbf{\phantom{0}9.45} & \phantom{0}93 & \textbf{\phantom{0,}590.33} & 47.56\\\midrule

% FAST & \phantom{0}2.63 & \phantom{0}1.91 & \phantom{0}53 & \phantom{0,}331.12 & \phantom{0} & 
%     \phantom{0}9.37 & \phantom{0}4.42 & \phantom{0}68 & \phantom{00,}191.27 & \phantom{0} & 
%     13.53 & \phantom{0}8.82 & 122 & \phantom{0,}869.57 & \phantom{0}\\
% FAST + Ours & \textbf{\phantom{0}1.73} & \textbf{\phantom{0}1.48} & \textbf{\phantom{0}50} & \textbf{\phantom{0,}185.23} & 44.06 & 
%     \textbf{\phantom{0}4.39} & \textbf{\phantom{0}3.37} & \textbf{\phantom{0}59} & \textbf{\phantom{00,0}97.63} & 48.96 & 
%     \textbf{\phantom{0}8.84} & \textbf{\phantom{0}7.18} & \textbf{118} & \textbf{\phantom{0,}602.64} & 30.70\\\midrule

% LOFTR & 24.52 & 16.16 & 194 & 4,808.87 & \phantom{0} & 
%     \textbf{10.14} & \textbf{\phantom{0}7.18} & 451 & 16,661.33 & \phantom{0} & 
%     \textbf{35.69} & 26.27 & 354 & 5,820.45 & \phantom{0}\\
% LOFTR + Ours & \textbf{21.62} & \textbf{14.24} & \textbf{189} & \textbf{3,227.65} & 32.88 & 
%     12.16 & \phantom{0}8.52 & \textbf{434} & \textbf{10,548.44} & 36.69 & 
%     37.30 & \textbf{26.20} & \textbf{337} & \textbf{4,287.66} & 26.33 \\\midrule

% ORB & \phantom{0}1.80 & \phantom{0}1.27 & \phantom{0}60 & \phantom{0,}512.54 & \phantom{0} & 
%     47.10 & 30.80 & \phantom{0}83 & \phantom{00,}492.19 & \phantom{0} & 
%     53.83 & 37.58 & \textbf{101} & \phantom{0,}654.07 & \phantom{0}\\
% ORB + Ours & \textbf{\phantom{0}1.47} & \textbf{\phantom{0}1.03} & \textbf{\phantom{0}59} & \textbf{\phantom{0,}281.84} & 45.01 & 
%     \textbf{35.58} & \textbf{22.90} & \textbf{\phantom{0}77} & \textbf{\phantom{00,}154.23} & 68.66 & 
%     \textbf{17.53} & \textbf{13.15} & 105 & \textbf{\phantom{0,}385.00} & 41.14\\\midrule

% SIFT & \phantom{0}4.00 & \phantom{0}2.92 & \textbf{\phantom{0}62} & \phantom{0,}480.22 & \phantom{0} & 
%     \phantom{0}6.57 & \phantom{0}3.37 & 185 & \phantom{0}1,205.78 & \phantom{0} & 
%     29.20 & 19.45 & \textbf{\phantom{0}58} & \phantom{0,}300.08 & \phantom{0} \\
% SIFT + Ours & \textbf{\phantom{0}1.82} & \textbf{\phantom{0}1.49} & \phantom{0}63 & \textbf{\phantom{0,}206.48} & 57.00 & 
%     \textbf{\phantom{0}2.69} & \textbf{\phantom{0}1.88} & \textbf{179} & \textbf{\phantom{00,}411.52} & 65.87 & 
%     \textbf{20.47} & \textbf{13.22} & \phantom{0}61 & \textbf{\phantom{0,}121.19} & 59.61\\\midrule

% SuperPoint & \phantom{0}1.75 & \phantom{0}1.41 & \textbf{\phantom{0}65} & \phantom{0,}355.84 & \phantom{0} & 
%     \phantom{0}4.29 & \phantom{0}2.43 & 133 & \phantom{0}1,708.62 & \phantom{0} & 
%     33.83 & 24.60 & 150 & \phantom{0,}534.23 & \phantom{0}\\
% SuperPoint + Ours & \textbf{\phantom{0}1.19} & \textbf{\phantom{0}0.89} & \phantom{0}69 & \textbf{\phantom{0,}213.34} & 40.04 & 
%     \textbf{\phantom{0}2.03} & \textbf{\phantom{0}1.60} & \textbf{133} & \textbf{\phantom{00,}972.46} & 43.09 & 
%     \textbf{27.63} & \textbf{20.68} & \textbf{148} & \textbf{\phantom{0,}355.84} & 33.39\\\midrule

% % SURF & 2.82 & 2.22 & \textbf{76} & 462.66 & \phantom{0} & 56.13 & 44.96 & \textbf{237} & 346.96 & \phantom{0} & -1.00 & -1.00 & -1.000 & -1.00 & -1.00\\
% % SURF + Ours & \textbf{1.22} & \textbf{1.07} & 77 & \textbf{207.16} & 55.22 & \textbf{38.49} & \textbf{23.81} & 238 & \textbf{\phantom{0}90.85} & 73.82 & -1.00 & -1.00 & -1.000 & -1.000 & -1.00\\\midrule

% Shi-Tomasi & 30.16 & \phantom{0}9.14 & \textbf{\phantom{0}15} & \phantom{0,}385.94 & \phantom{0} & 
%     43.18 & 27.07 & \textbf{\phantom{0}14} & \phantom{00,}497.58 & \phantom{0} & 
%     28.95 & 19.30 & \textbf{\phantom{0}28} & 1,415.69 & \phantom{0}\\
% Shi-Tomasi + Ours & \textbf{\phantom{0}3.66} & \textbf{\phantom{0}2.65} & \textbf{\phantom{0}15} & \textbf{\phantom{0,}148.88} & 61.42 & 
%     \textbf{39.97} & \textbf{26.76} & \textbf{\phantom{0}14} & \textbf{\phantom{00,}155.62} & 68.72 & 
%     \textbf{22.36} & \textbf{15.64} & \phantom{0}31 & \textbf{\phantom{0,}898.84} & 36.51\\\midrule

% SILK & 37.25 & 18.90 & \textbf{382} & \phantom{0,}441.82 & \phantom{0} & 
%     55.74 & 37.51 & 590 & \phantom{00,}676.29 & \phantom{0} & 
%     33.07 & 23.03 & \textbf{375} & \phantom{0,}674.15 & \phantom{0}\\
% SILK + Ours & \textbf{20.40} & \textbf{15.10} & \textbf{382} & \textbf{\phantom{0,}217.30} & 50.82 & 
%     \textbf{51.33} & \textbf{35.56} & \textbf{588} & \textbf{\phantom{00,}168.75} & 75.05 & 
%     \textbf{31.90} & \textbf{22.65} & 376 & \textbf{\phantom{0,}292.55} & 56.60\\\bottomrule

% \end{tabular}
% }
% \caption{Visual odometry (VO) performance results. Features when filtered using \qq{} contribute to a lower RMSE (31\% on average across all datasets), MAE, and frame-to-frame execution time for VO estimation (0.63\% despite the inclusion of model inference). This enables using lighter, faster features like Shi-Tomasi while achieving performance better than SIFT (e.g., KITTI \& Davis). We see a considerable reduction in the number of keypoints in all datasets by roughly 49\% (\(mean (|KP|\downarrow\)) shows \% reduction while $mean(|KP|)$ shows the mean number of keypoints extracted per image). $mean(F_\text{Area})$ is the average percentage of pixels masked with $F$.}
% \label{tab:vo-eval}
% \end{table*}


==> sections/tables/in-out.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{graphicx}
% \begin{table}[]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}l|lllll|lllll@{}}
% \toprule
% Feature              & \multicolumn{5}{c|}{KITTI}                           & \multicolumn{5}{c}{CODa}                             \\ \midrule
%                      & \(|kps|\) & \(\mu_{inliers}\) & \(\sigma_{inliers}\) & \(\mu_{outliers}\) & \(\sigma_{outliers}\) & \(|kps|\) & \(\mu_{inliers}\) & \(\sigma_{inliers}\) & \(\mu_{outliers}\) & \(\sigma_{outliers}\) \\ \midrule
% Brisk                & 752      & 488      & 159     & 264       & 50       & 568      & 445      & 251     & 123       & 66       \\
% Brisk + Ours         & 343      & 229      & 104     & 114       & 39       & 181      & 142      & 62      & 39        & 30       \\ \midrule
% FAST                 & 331      & 176      & 76      & 155       & 30       & 191      & 136      & 106     & 55        & 26       \\
% FAST + Ours          & 185      & 102      & 49      & 83        & 22       & 98       & 70       & 47      & 28        & 18       \\ \midrule
% LOFTR                &          &          &         &           &          &          &          &         &           &          \\
% LOFT + Ours          &          &          &         &           &          &          &          &         &           &          \\ \midrule
% ORB                  & 513      & 290      & 134     & 222       & 64       & 492      & 375      & 281     & 118       & 64       \\
% ORB + Ours           & 282      & 164      & 87      & 118       & 43       & 154      & 113      & 66      & 41        & 33       \\ \midrule
% SIFT                 & 480      & 391      & 104     & 89        & 26       & 1206     & 1064     & 384     & 142       & 89       \\
% SIFT + Ours          & 206      & 170      & 67      & 37        & 16       & 412      & 358      & 140     & 53        & 47       \\ \midrule
% Superpoint           & 356      & 178      & 43      & 178       & 23       & 1709     & 1007     & 445     & 702       & 250      \\
% Superpoint + Ours    & 213      & 106      & 33      & 107       & 22       & 972      & 560      & 223     & 412       & 152      \\ \midrule
% SURF                 & 463      & 311      & 114     & 151       & 31       & 347      & 300      & 86      & 47        & 29       \\
% SURF + Ours          & 207      & 140      & 59      & 67        & 21       & 91       & 77       & 33      & 14        & 14       \\ \midrule
% LK_SHI_TOMASI        & 386      & 320      & 43      & 66        & 36       & 498      & 478      & 41      & 19        & 35       \\
% LK_SHI_TOMASI + Ours & 149      & 122      & 38      & 27        & 19       & 156      & 147      & 46      & 8         & 22       \\ \bottomrule
% \end{tabular}%
% }
% \caption{todo}
% \label{tab:in-out}
% \end{table}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[htbp]
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}l|lllll|lllll@{}}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{Feature}} & \multicolumn{5}{c|}{KITTI}                           & \multicolumn{5}{c}{CODa}                             \\ \cmidrule(l){2-11} 
\multicolumn{1}{c|}{}                         & \(|kps|\) & \(\mu_{inliers}\) & \(\sigma_{inliers}\) & \(\mu_{outliers}\) & \(\sigma_{outliers}\) & \(|kps|\) & \(\mu_{inliers}\) & \(\sigma_{inliers}\) & \(\mu_{outliers}\) & \(\sigma_{outliers}\) \\ \midrule
Brisk                                         & 752      & 488      & 159     & 264       & 50       & 568      & 445      & 251     & 123       & 66       \\
Brisk + Ours                                  & 343      & 229      & 104     & 114       & 39       & 181      & 142      & 62      & 39        & 30       \\ \midrule
FAST                                          & 331      & 176      & 76      & 155       & 30       & 191      & 136      & 106     & 55        & 26       \\
FAST + Ours                                   & 185      & 102      & 49      & 83        & 22       & 98       & 70       & 47      & 28        & 18       \\ \midrule
LOFTR                                         &          &          &         &           &          &          &          &         &           &          \\
LOFT + Ours                                   &          &          &         &           &          &          &          &         &           &          \\ \midrule
ORB                                           & 513      & 290      & 134     & 222       & 64       & 492      & 375      & 281     & 118       & 64       \\
ORB + Ours                                    & 282      & 164      & 87      & 118       & 43       & 154      & 113      & 66      & 41        & 33       \\ \midrule
SIFT                                          & 480      & 391      & 104     & 89        & 26       & 1206     & 1064     & 384     & 142       & 89       \\
SIFT + Ours                                   & 206      & 170      & 67      & 37        & 16       & 412      & 358      & 140     & 53        & 47       \\ \midrule
Superpoint                                    & 356      & 178      & 43      & 178       & 23       & 1709     & 1007     & 445     & 702       & 250      \\
Superpoint + Ours                             & 213      & 106      & 33      & 107       & 22       & 972      & 560      & 223     & 412       & 152      \\ \midrule
SURF                                          & 463      & 311      & 114     & 151       & 31       & 347      & 300      & 86      & 47        & 29       \\
SURF + Ours                                   & 207      & 140      & 59      & 67        & 21       & 91       & 77       & 33      & 14        & 14       \\ \midrule
LK\_SHI\_TOMASI                                 & 386      & 320      & 43      & 66        & 36       & 498      & 478      & 41      & 19        & 35       \\
LK\_SHI\_TOMASI + Ours                          & 149      & 122      & 38      & 27        & 19       & 156      & 147      & 46      & 8         & 22       \\ \bottomrule
\end{tabular}%
% }
\caption{Feature Matching Performance: The reduction in keypoints following feature filtering with \qq{} directly impacts RANSAC matching performance. Notably, we observe a significant decrease in outliers during this process. This improvement can be attributed to the inherent stability and robustness of features extracted from regions identified as high featureness by \qq{}. While the overall number of inliers also decreases due to the reduced feature count, this reduction has no detrimental effect on downstream performance. }
\label{tab:in-out}
\end{table*}

==> sections/tables/silk_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[]
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}l|cccccc|cccccc|cccccc@{}}
\toprule
\multirow{2}{*}{Feature} & \multicolumn{6}{c|}{\textbf{KITTI} ($\mu F_\text{Area}$: 30.98\%)}         & \multicolumn{6}{c|}{\textbf{CODa} ($\mu F_\text{Area}$: 33.65\%)}             & \multicolumn{6}{c}{\textbf{Davis} ($\mu F_\text{Area}$: 66.21\%)}       \\ \cmidrule(l){2-19} 
& \multicolumn{1}{l}{RMSE} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{$t_{VO}$} & \multicolumn{1}{l}{$t_{Total}$} & \multicolumn{1}{l}{$\mu_{|Kp|}$} & \multicolumn{1}{l|}{$|Kp|\downarrow$} & \multicolumn{1}{l}{RMSE} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{$t_{VO}$} & \multicolumn{1}{l}{$t_{Total}$} & \multicolumn{1}{l}{$\mu_{|Kp|}$} & \multicolumn{1}{l|}{$|Kp|\downarrow$} & \multicolumn{1}{l}{RMSE} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{$t_{VO}$} & \multicolumn{1}{l}{$t_{Total}$} & \multicolumn{1}{l}{$\mu_{|Kp|}$} & \multicolumn{1}{l}{$|Kp|\downarrow$} \\ \midrule
Brisk & \phantom{0}1.78 & \textbf{1.17 } & 0.060 & \textbf{0.060 } & 752.34 & 0.00 & 46.64 & 34.27 & 0.116 & 0.116 & 567.94 & 0.00 & 32.63 & 23.92 & 0.091 & \textbf{0.091} & 1,125.75 & 0.00 \\
Brisk + Ours             & \textbf{1.547 }                   & 1.27                    & \textbf{0.058 }                      & \textbf{0.060}    & \textbf{342.89}                      & 54.42                       & \textbf{46.33 }                   & \textbf{30.64}                   & \textbf{0.112 }                      & \textbf{0.114}    & \textbf{180.81}                      & 68.20                       & \textbf{13.10 }                   & \textbf{9.45}                    & 0.092                       & 0.093    & \textbf{590.33}                      & 47.56                      \\ \midrule
FAST                     & 2.631                    & 1.91                    & 0.053                       & 0.053    & 331.12                      & 0.00                        & 9.37                     & 4.42                    & 0.068                       & 0.068    & 191.27                      & 0.00                        & 13.53                    & 8.82                    & 0.122                       & 0.122    & 869.57                      & 0.00                       \\
FAST + Ours              & \textbf{1.731}                    & \textbf{1.48  }                  & \textbf{0.048}                       & \textbf{0.050}    & \textbf{185.23}                      & 44.06                       & \textbf{4.39}                     & \textbf{3.37}                    & \textbf{0.057}                       & \textbf{0.059}    & \textbf{97.63}                       & 48.96                       & \textbf{8.84 }                    & \textbf{7.18 }                   & \textbf{0.117 }                      & \textbf{0.118}    & \textbf{602.64}                      & 30.70                      \\ \midrule
LOFTR                    & 24.52                       & 16.16                      & 0.194                      & 0.194   & 4808.87                       & 0                       & \textbf{10.14}                       & \textbf{7.18}                     & 0.451                      & 0.451   & 16661.33                       & 0.00                       & \textbf{35.69}                    & 26.27                   & 0.354                       & 0.354    & 5,820.45                    & 0.00                       \\
LOFT + Ours              & \textbf{21.62}                       & \textbf{14.24}                      & \textbf{0.187}                      & \textbf{0.189}   & \textbf{3227.65}                       & 32.88                       & 12.16                       & 8.52                      & \textbf{0.432}                      & \textbf{0.434}   & \textbf{10548.44}                       & 36.69                       & 37.30                    & \textbf{26.20}                   & \textbf{0.335 }                      & \textbf{0.337}    & \textbf{4,287.66}                    & 26.33                      \\ \midrule
ORB                      & 1.802                    & 1.27                    & 0.060                       & 0.060    & 512.54                      & 0.00                        & 47.1                     & 30.8                    & 0.083                       & 0.083    & 492.19                      & 0.00                        & 53.83                    & 37.58                   & \textbf{0.101}                       & \textbf{0.101}    & 654.07                      & 0.00                       \\
ORB + Ours               & \textbf{1.469}                    & \textbf{1.03}                    & \textbf{0.057}                       & \textbf{0.059}    & \textbf{281.84}                      & 45.01                       & \textbf{35.58}                    & \textbf{22.9}                    & \textbf{0.075}                       & \textbf{0.077}    & \textbf{154.23 }                     & 68.66                       & \textbf{17.53}                    & \textbf{13.15}                   & 0.103                       & 0.105    & \textbf{385.00}                      & 41.14                      \\ \midrule
SIFT                     & 3.996                    & 2.92                    & 0.062                       & \textbf{0.062 }   & 480.22                      & 0.00                        & 6.57                     & 3.37                    & 0.185                       & 0.185    & 1,205.78                    & 0.00                        & 29.20                    & 19.45                   & \textbf{0.058}                       & \textbf{0.058}    & 300.08                      & 0.00                       \\
SIFT + Ours              & \textbf{1.817}                    & \textbf{1.49}                    & \textbf{0.061}                       & 0.063    & \textbf{206.48 }                     & 57.00                       & \textbf{2.69}                     & \textbf{1.88 }                   & \textbf{0.177}                       & \textbf{0.179}    & \textbf{411.52}                      & 65.87                       & \textbf{20.47}                    & \textbf{13.22}                   & 0.059                       & 0.061    & \textbf{121.19}                      & 59.61                      \\ \midrule
Superpoint               & 1.745                    & 1.41                    & \textbf{0.065}                       & \textbf{0.065}    & 355.84                      & 0.00                        & 4.29                     & 2.43                    & \textbf{0.133}                       & 0.133    & 1,708.62                    & 0.00                        & 33.83                    & 24.60                   & 0.150                       & 0.150    & 534.23                      & 0.00                       \\
Superpoint + Ours        & \textbf{1.188}                    & \textbf{0.89}                    & 0.067                       & 0.069    & \textbf{213.34}                      & 40.04                       & \textbf{2.03}                     & \textbf{1.6}                     & \textbf{0.131}                       & \textbf{0.133}    & \textbf{972.46}                      & 43.09                       & \textbf{27.63 }                   & \textbf{20.68}                   & \textbf{0.146}                       & \textbf{0.148}    & \textbf{355.84}                      & 33.39                      \\ \midrule
SURF                     & 2.816                    & 2.22                    & 0.076                       & \textbf{0.076}    & 462.66                      & 0.00                        & 56.13                    & 44.96                   & 0.237                       & \textbf{0.237}    & 346.96                      & 0.00                        & -1.00                    & -1.00                   & -1.000                      & -1.000   & -1.00                       & -1.00                      \\
SURF + Ours              & \textbf{1.218}                    & \textbf{1.07}                    & \textbf{0.074}                       & 0.077    & \textbf{207.16}                      & 55.22                       & \textbf{38.49}                    & \textbf{23.81}                   & \textbf{0.236}                       & 0.238    & \textbf{90.85}                       & 73.82                       & -1.00                    & -1.00                   & -1.000                      & -1.000   & -1.00                       & -1.00                      \\ \midrule
Shi\_Tomasi          & 30.16                    & 9.14                    & 0.015                       &\textbf{ 0.015}    & 385.94                      & 0.00                        & 43.18                    & 27.07                   & 0.014                       & \textbf{0.014}    & 497.58                      & 0.00                        & 28.95                    & 19.30                   & \textbf{0.028}                       & \textbf{0.028}    & 1,415.69                    & 0.00                       \\
Shi\_Tomasi + Ours   & \textbf{3.66}                     & \textbf{2.65}                    & \textbf{0.013}                      & \textbf{0.015}    & \textbf{148.88}                      & 61.42                       & \textbf{39.97}                    & \textbf{26.76}                   & \textbf{0.012}                       & \textbf{0.014}    & \textbf{155.62}                      & 68.72                       & \textbf{22.36}                    & \textbf{15.64}                   & 0.029                       & 0.031    & \textbf{898.84}                      & 36.51                      \\ \midrule
SILK                     & 37.25                    & 18.9                    & 0.382                     & \textbf{0.382}    & 441.82                      & 0.00                        & 55.74                       & 37.51                      & 0.590                      & 0.590   & 676.29                       & 0                       & 33.07                    & 23.03                   & \textbf{0.375}                       & \textbf{0.375}    & 674.15                      & 0.00                       \\
SILK + Ours              & \textbf{20.4}                     & \textbf{15.1}                    & \textbf{0.380}                       & \textbf{0.382}    & \textbf{217.30}                      & 50.82                       & \textbf{51.33}                       & \textbf{35.56}                     & \textbf{0.586}                      & \textbf{0.588}   & \textbf{168.75}                       & 75.05                       & \textbf{31.90}                    & \textbf{22.65}                   & \textbf{0.375}                       & 0.376    & \textbf{292.55}                      & 56.60                      \\ \bottomrule
\end{tabular}
}
\caption{Visual-odometry (VO) performance results. Features when filtered using \qq{} contribute to a lower RMSE, MAE and execution time for VO estimation. This enables using lighter, faster features like Shi-Tomasi while achieving performance better than SIFT (Eg. KITTI \& Davis).We see a considerable reduction in number of key-points, (\(|kp|\downarrow\) shows \% reduction)}
\label{tab:vo-eval2}
\end{table*}
